Out of Sight Out of Mind, Out of Sight Out of Mind: Measuring Bias in Language Models Against Overlooked Marginalized Groups in Regional Contexts

We know that language models (LMs) form biases and stereotypes of minorities, leading to unfair treatments of members of these groups, thanks to research mainly in the US and the broader English-speaking world. As the negative behavior of these models has severe consequences for society and individuals, industry and academia are actively developing methods to reduce the bias in LMs. However, there are many under-represented groups and languages that have been overlooked so far. This includes marginalized groups that are specific to individual countries and regions in the English speaking and Western world, but crucially also almost all marginalized groups in the rest of the world. The UN estimates, that between 600 million to 1.2 billion people worldwide are members of marginalized groups and in need for special protection. If we want to develop inclusive LMs that work for everyone, we have to broaden our understanding to include overlooked marginalized groups and low-resource languages and dialects. In this work, we contribute to this effort with the first study investigating offensive stereotyping bias in 23 LMs for 270 marginalized groups from Egypt, the remaining 21 Arab countries, Germany, the UK, and the US. Additionally, we investigate the impact of low-resource languages and dialects on the study of bias in LMs, demonstrating the limitations of current bias metrics, as we measure significantly higher bias when using the Egyptian Arabic dialect versus Modern Standard Arabic. Our results show, LMs indeed show higher bias against many marginalized groups in comparison to dominant groups. However, this is not the case for Arabic LMs, where the bias is high against both marginalized and dominant groups in relation to religion and ethnicity. Our results also show higher intersectional bias against Non-binary, LGBTQIA+ and Black women.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> backup.tex <==
\subsection{HONEST Detailed Results per Gender and Intersectional Analysis}
\label{appx:honest_details}

\begin{table}[h!]
\centering
\small
\begin{tabular}{
    l  % Model
    S S S % ar: female, male, nonbinary
    S S S % ar-eg
    S S S % de
    S S S % en-uk
    S S S % en-us
}
\toprule
& \multicolumn{3}{c}{ar} & \multicolumn{3}{c}{ar-eg} & \multicolumn{3}{c}{de} & \multicolumn{3}{c}{en-uk} & \multicolumn{3}{c}{en-us} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
\multirow{2}{*}{\textbf} & \multicolumn{1}{c}{fem} & \multicolumn{1}{c}{male} & \multicolumn{1}{c}{nonb} & \multicolumn{1}{c}{fem} & \multicolumn{1}{c}{male} & \multicolumn{1}{c}{nonb} & \multicolumn{1}{c}{fem} & \multicolumn{1}{c}{male} & \multicolumn{1}{c}{nonb} & \multicolumn{1}{c}{fem} & \multicolumn{1}{c}{male} & \multicolumn{1}{c}{nonb} & \multicolumn{1}{c}{fem} & \multicolumn{1}{c}{male} & \multicolumn{1}{c}{nonb}\\
\midrule
\multirow{1}{*}{bloom-7b1} 
 & 11.7926 & 11.1602 & 10.5731  & 11.5126 & 12.3    & 11.4699 & 1.3042 & 2.0562 & 0.81455 & 26.2979 & 26.9596 & 28.1577 & 26.0111 & 26.0111 & 27.5926 \\

\multirow{1}{*}{Llama-3.1-8B} 
 & 5.9583  & 6.6306  & 6.2963   & 4.2225  & 4.2990  & 6.6038  & 3.1384 & 2.6542 & 3.7421  & 23.5140 & 24.8183 & 27.8131 & 23.0028 & 23.0028 & 26.6195 \\

\multirow{1}{*}{aya-expanse-8b} 
 & 5.0852  & 5.4250  & 6.1759   & 6.9685  & 6.8999  & 6.4874  &      &      &        & 21.9467 & 22.9770 & 26.0487 & 22.3544 &       & 25.7992 \\


\multirow{1}{*}{flan-t5-base}
 & 0.0148   & 0.0074   & 0.0694    & 0.0154  & 0.0      & 0.0926   & 0.9196 & 1.6518 & 1.7401  & 5.8689  & 4.8355  & 7.5932   & 6.1782  & 5.6462  & 6.8258  \\

\multirow{1}{*}{gpt-4}
 & 0.3194   & 0.1963   & 0.0889    & 0.5401  & 0.6612  & 0.3757   & 0.0    & 0.02551 & 0.02232 & 0.3768  & 0.3097  & 0.6225   & 0.3996  & 0.3642  & 0.8014  \\
 \hline
 
 \multirow{1}{*}{AceGPT-13B}
 & 3.7852  & 4.2861  & 3.9185   & 4.3738  & 5.6413  & 4.7492  &      &      &        &       &       &        &       &       &        \\

  \multirow{1}{*}{Jais-13B}
 & 3.7852  & 4.2861  & 3.9185   & 4.3738  & 5.6413  & 4.7492  &      &      &        &       &       &        &       &       &        \\
 \hline
 \multirow{1}{*}{LLaMmlein\_1B}
 &        &        &         &        &        &        & 2.6709 & 3.6936 & 3.0146  &       &       &        &       &       &        \\

\multirow{1}{*}{Leo-mistral}
 &        &        &         &        &        &        & 1.9653 & 2.0736 & 2.6826  &       &       &        &       &       &        \\
\bottomrule
\end{tabular}
\caption{Percentages by Model (rows), Language (grouped columns), and Gender (subcolumns). Blank cells indicate no data.}
\end{table}


\begin{table}[h!]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Attribute} & \textbf{Max Difference} & \textbf{Mean Difference} & \textbf{Variance} \\
\midrule
Gender            & 2.41 & -0.94 & 3.55 \\
Physical Ability  & 5.77 &  0.42 & 4.82 \\
ethnicity              & 7.04 & -3.01 & 78.84 \\
Refugees          & 2.50 & -0.45 & 3.81 \\
Religion          & 4.33 & -0.12 & 3.06 \\
Sexual Orientation & 14.65 & -0.03 & 22.99 \\
\bottomrule
\end{tabular}
\caption{Aggregated Intersectional Differences of HONEST by Attribute}
\label{tab:intersectional_differences}
\end{table}

\begin{figure}[h!]
    \centering
    
    \begin{subfigure}{0.49\textwidth}
    \Description{The graph displays HONEST scores (in percent), ranging from 0 to 20\% across five sensitive attributes: Gender, Disability, Race, Religion, and Sexual Orientation. Data points are grouped by model, represented with different marker styles and colors: Llama-3.1-8B, aya-expanse-8b, bloom-7b1, flan-t5-base, and gpt-4. Gender is further visualized using different shapes: nonbinary, female, and male. The scores vary widely across models and attributes. Higher scores are generally observed for Disability Race and Religion for the bloom-7b1 model, while lower scores appear for Gender and Sexual Orientation and the flan-t5-base and gpt-4 model.}
        \caption{Egyptian}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/Davids_plots/AR-EG.png}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph displays HONEST scores (in percent), ranging from 0 to 25\% across five sensitive attributes: Gender, Disability, Race, Religion, and Sexual Orientation. Data points are grouped by model, represented with different marker styles and colors: LlaMmlein_1B, Llama-3.1-8B, bloom-7b1, flan-t5-base, and gpt-4. Gender is further visualized using different shapes: nonbinary, female, and male. The scores vary widely across models and attributes. Higher scores are generally observed for Disability and Sexual Orientation for the LlaMmlein_1B, Llama-3.1-8b and leo-mistral-hessianai-7b-chat model, while lower scores appear for Gender, Race and Religion and the gpt-4 model.}
        \caption{German}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/Davids_plots/GE.png}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph displays HONEST scores (in percent), ranging from 0 to 45\% across five sensitive attributes: Gender, Disability, Race, Religion, and Sexual Orientation. Data points are grouped by model, represented with different marker styles and colors: Llama-3.1-8B, aya-expanse-8b, bloom-7b1, flan-t5-base, and gpt-4. Gender is further visualized using different shapes: nonbinary, female, and male. The scores vary widely across models and attributes. Higher scores are generally observed for Sexual Orientation for the Llama-3.1.-8B model, while lower scores appear for Gender, Disability, Race and Religion and the flan-t5-base and gpt-4 model.}
        \caption{English UK}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/Davids_plots/UK_HONEST.png}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph displays HONEST scores (in percent), ranging from 0 to 45\% across five sensitive attributes: Gender, Disability, Race, Religion, and Sexual Orientation. Data points are grouped by model, represented with different marker styles and colors: Llama-3.1-8B, aya-expanse-8b, bloom-7b1, flan-t5-base, and gpt-4. Gender is further visualized using different shapes: nonbinary, female, and male. The scores vary widely across models and attributes. Higher scores are generally observed for Race and Sexual Orientation for the Llama-3.1.-8B model, while lower scores appear for Gender, Disability adn Religion and the flan-t5-base and gpt-4 model.}
        \caption{English US}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/Davids_plots/US.png}
    \end{subfigure}
    \caption{Results HONEST scores grouped by sensitive attributes for all three genders}
    \label{fig:enter-label}
\end{figure}
\newpage
\FloatBarrier
\subsection{HONEST Detailed Results Identities in Regional Contexts}
 
\newpage
\newpage

\begin{figure}[h!]
     \centering
    \Description{The graph displays the mean HONEST score in percentage across five sensitive attributes: Religion, Physical Ability, Ethnicity, Sexual Orientation, and Gender. The y-axis represents the mean HONEST score in percentage, ranging from 0 to 16\%. The x-axis categorizes the data by sensitive attributes. Two groups are visualized: Dominant and Marginalized, each with a boxplot in the background. Each group is represented with markers for different models: bloom-7b1, gpt-4, flan-t5-base, Llama-3.1-8B, and aya-expanse-8b. Dominant group markers are circular, square, diamond, upward triangle, and downward triangle, while Marginalized group markers use the same shapes but in green. The plot shows variation in scores, with marginalized groups often showing higher values compared to dominant groups across categories. Religion and Sexual Orientation exhibit lower overall scores, while Ethnicity and Gender display greater variation. A legend in the upper-right corner labels the marker types by model and group.}
    \includegraphics[width=0.8\textwidth]{figures/Generative_models/Arabic/MSA/Bias_ar_withBox.png}
    \label{fig:arab_HONEST}
    \caption{The distribution of HONEST scores per sensitive attribute and model for marginalized groups plotted against dominant groups in the Arab world.}
\end{figure}

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Circassian, Benadiri and Black being in the beginning. The y-axis represents HONEST scores, ranging from 0 to 14\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Circassian and Muhamash having higher HONEST scores for females while others like Black and Armenian have a more uniform distribution across genders. Male is the gender with the highest HONEST Score for most categories.}
        \caption{The distribution of HONEST scores per sensitive attribute and model for marginalized groups plotted against dominant groups in the Arab world.}
        \includegraphics[width = \textwidth]{figures/Generative_models/Arabic/MSA/Bias_ar_withBox.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Buddhist, Samaritan and Islamili at the beginning. The y-axis represents HONEST scores, ranging from 0 to 10\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Buddhist and Jewish having higher HONEST scores for nonbinary while others like Samaritan and Coptic have a more uniform distribution across genders. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{The distribution of HONEST scores per sensitive attribute and model for marginalized groups plotted against dominant groups in Egypt.}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/Davids_plots/BIAS_EG.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Yazidi, Hindu and Jewish at the beginning. The y-axis represents HONEST scores, ranging from 0 to 14\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Hindu and Christian having higher HONEST scores for nonbinary while others like Yazidi and Coptic have a more uniform distribution across genders. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{The distribution of HONEST scores per sensitive attribute and model for marginalized groups plotted against dominant groups in Germany.}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/Davids_plots/BIAS_GE.png}
    \end{subfigure} 
    \hfill
    %Egyptian
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Berber, Black and Arab at the beginning. The y-axis represents HONEST scores, ranging from 0 to 35\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Berber and Amazighi having a uniform distribution across genders and others like Black and Gypsy having overlapping HONEST Scores for different genders. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{The distribution of HONEST scores per sensitive attribute and model for marginalized groups plotted against dominant groups in the US.}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/Davids_plots/BIAS_US.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with South-Sudanise, Iraqui and Syrian at the beginning. The y-axis represents HONEST scores, ranging from 0 to 10\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Iraqui and Eritrean having higher HONEST scores for nonbinary while others like Syrian and Ethopian have a more uniform distribution across genders. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{The distribution of HONEST scores per sensitive attribute and model for marginalized groups plotted against dominant groups in the UK.}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/Davids_plots/BIAS_UK.png}
    \end{subfigure} 

    \end{figure}

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Circassian, Benadiri and Black being in the beginning. The y-axis represents HONEST scores, ranging from 0 to 14\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Circassian and Muhamash having higher HONEST scores for females while others like Black and Armenian have a more uniform distribution across genders. Male is the gender with the highest HONEST Score for most categories.}
        \caption{Arabic AceGPT-13-B Race}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/ar_AceGPT-13B_Race.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Buddhist, Samaritan and Islamili at the beginning. The y-axis represents HONEST scores, ranging from 0 to 10\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Buddhist and Jewish having higher HONEST scores for nonbinary while others like Samaritan and Coptic have a more uniform distribution across genders. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{Arabic AceGPT-13B Religion}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/ar_AceGPT-13B_Religion.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Yazidi, Hindu and Jewish at the beginning. The y-axis represents HONEST scores, ranging from 0 to 14\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Hindu and Christian having higher HONEST scores for nonbinary while others like Yazidi and Coptic have a more uniform distribution across genders. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{Arabic Llama-3.1-8B Religion}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/ar_Llama-3.1-8B_Religion.png}
    \end{subfigure} 
    \hfill
    %Egyptian
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Berber, Black and Arab at the beginning. The y-axis represents HONEST scores, ranging from 0 to 35\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Berber and Amazighi having a uniform distribution across genders and others like Black and Gypsy having overlapping HONEST Scores for different genders. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{Egpytian Llama-3.1-8B Race}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/ar-eg_Llama-3.1-8B_Race.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with South-Sudanise, Iraqui and Syrian at the beginning. The y-axis represents HONEST scores, ranging from 0 to 10\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Iraqui and Eritrean having higher HONEST scores for nonbinary while others like Syrian and Ethopian have a more uniform distribution across genders. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{Egpytian Llama-3.1-8B Refugee}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/ar-eg_Llama-3.1-8B_Refugee.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Shi'a, Sufi and without-Religion at the beginning. The y-axis represents HONEST scores, ranging from 0 to 10\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Shi'a and Sufi having higher HONEST scores for nonbinary and female. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{Egpytian Llama-3.1-8B Religion}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/ar-eg_Llama-3.1-8B_Religion.png}
    \end{subfigure} 
    \hfill
    %German
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with German, Russian and Ukrainian at the beginning. The y-axis represents HONEST scores, ranging from 0 to 3.5\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with the German category being evenly distributed and the others having overlapping HONEST Scores for the same gender. Nonbinary and male are the genders with the highest HONEST Score for most categories.}
        \caption{German Leo-Mistral-Hessianai-7b-chat Refugees}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/de_leo-mistral-hessianai-7b-chat_Refugees.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Non-religious, Buddhist and Agnostic at the beginning. The y-axis represents HONEST scores, ranging from 0 to 3.5\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with the Non-religious, Muslim and Catholic categories being evenly distributed and the others having overlapping HONEST Scores for the same gender. Nonbinary and male are the genders with the highest HONEST Score for most categories.}
         \caption{German Leo-Mistral-Hessianai-7b-chat Religion}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/de_leo-mistral-hessianai-7b-chat_Religion.png}
    \end{subfigure}
\end{figure}

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Gay, Homosexual and Heterosexual at the beginning. The y-axis represents HONEST scores, ranging from 0 to 14\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores vary across identities, with some groups such as Gay and Heterosexual having higher HONEST scores for nonbinary while others like Homosexual and Asexual have a more uniform distribution across genders. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{German Leo-Mistral-Hessianai-7b-chat Sexual Orientation}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/de_leo-mistral-hessianai-7b-chat_Sexual orientation.png}
    \end{subfigure} 
    \hfill
    %English UK
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with white, Black and Gypsy at the beginning. The y-axis represents HONEST scores, ranging from 0 to 55\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores have overlapping HONEST Scores for each category for male and female gender. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{English UK Aya-expanse-8b Race}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/en-uk_aya-expanse-8b_Race.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Hindu, Christian and Catholic at the beginning. The y-axis represents HONEST scores, ranging from 0 to 28\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores have overlapping HONEST Scores for each category for male and female gender. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{English UK Aya-expanse-8b Religion}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/en-uk_aya-expanse-8b_Religion.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Straight, Heterosexual and Homosexual at the beginning. The y-axis represents HONEST scores, ranging from 0 to 55\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores have overlapping HONEST Scores for each category for male and female gender. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{English UK Aya-expanse-8b Sexual Orientation}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/en-uk_aya-expanse-8b_Sexual-Orientation.png}
    \end{subfigure} 
    \hfill
    %English US
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Black, White and African at the beginning. The y-axis represents HONEST scores, ranging from 0 to 45\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores have overlapping HONEST Scores for each category for male and female gender. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{English US Bloom-7b1 Race}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/en-us_bloom-7b1_Race.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Muslim, Christian and Catholic at the beginning. The y-axis represents HONEST scores, ranging from 0 to 30\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores have overlapping HONEST Scores for each category for male and female gender. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{English US Bloom-7b1 Religion}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/en-us_bloom-7b1_Religion.png}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \Description{The graph shows HONEST scores (in percent) for various identities along the x-axis, ordered from highest to lowest mean score with Homosexual, Heterosexual and Gay at the beginning. The y-axis represents HONEST scores, ranging from 0 to 45\%. Data points are categorized by gender identity: nonbinary, male, and female. The scores have overlapping HONEST Scores for each category for male and female gender. Nonbinary is the gender with the highest HONEST Score for most categories.}
        \caption{English US Bloom-7b1 Sexual Orientation}
        \includegraphics[width = \textwidth]{figures/Generative_models/Appendix/en-us_bloom-7b1_Sexual-Orientation.png}
    \end{subfigure}
\end{figure}



\FloatBarrier
\subsection{Detailed MLM results for all models and individual identities}
\label{appx:detailed_results_MLM}
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.7\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/Arab_countries/SOS bias scores for all models displays senstive attribues.png}
       %  \caption{$y=x$}
       %  \label{fig:y equals x}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.7\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/Egypt/SOS bias scores for all models displays senstive attribues.png}
       %  \caption{$y=3\sin x$}
       %  \label{fig:three sin x}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.7\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/Germany/SOS bias scores for all models displays senstive attribues.png}
       %  \caption{$y=5/x$}
       %  \label{fig:five over x}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.7\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/UK/SOS bias scores for all models displays senstive attribues.png}
       %  \caption{$y=5/x$}
        % \label{fig:five over x}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.7\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/US/SOS bias scores for all models displays senstive attribues.png}
      %   \caption{$y=5/x$}
      %   \label{fig:five over x}
     \end{subfigure}
        \caption{The distribution of $SOS_{MLM}$ bias scores in the inspected models against marginalized and dominant identities in the different countries and for the different sensitive attributes.}
\end{figure}
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.7\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/Egypt/SOS bias scores for different gender refugees.png}
       %  \caption{$y=x$}
       %  \label{fig:y equals x}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.7\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/Germany/SOS bias scores for different gender refugees.png}
       %  \caption{$y=3\sin x$}
       %  \label{fig:three sin x}
     \end{subfigure}
        \caption{Heatmap of the $SOS_{MLM}$ bias scores against the refugees/nationals in Germany and Egypt.}
        \label{fig:heatmap-sos-refugees-all-gender}
\end{figure}
\begin{table}[h]
\footnotesize
\renewcommand{\arraystretch}{1.2}
     \resizebox{1\textwidth}{!}{
\begin{tabular}{c|ll}

\hline
            & \multicolumn{1}{c|}{Religion}                                                & \multicolumn{1}{c}{Ethnicity}                           \\ \hline
Arab world & \multicolumn{1}{l|}{Qurani, \underline {Sunni}, Christian, Yazidi, Ismaili}               & \underline {Arab}, Black, Armenian, South-Sudanese, Bantoy       \\ \hline

%Egypt & \multicolumn{1}{l|}{\underline {Sunni}, Qurani, Without-religion, Christian, Agnostic}               &  Bedouin, Amazighi, \underline {Arab}, Black, Nubian       \\ \hline

The US      & \multicolumn{1}{l|}{Druze, Jehova's witness, Buddhist, \underline{Catholic}, Unitarians} & Arab-American,  Haitian, \underline{Caucasian}, African, Latino \\ 
\hline
\hline
            
Arab world (HONEST)& \multicolumn{1}{l|}{Buddhist, Sufi, Hindu, Durzi, Yazidi}                      & Black, Berber, Armenians, Armenian, Circassian            \\ \hline
The US (HONEST)   & \multicolumn{1}{l|}{Agnostic, Atheist, \underline{Christian}, Muslim, \underline{Catholic}}  & Black, \underline{White}, African-American, Latino, Haitian       \\
%The UK      & \multicolumn{1}{l|}{Buddhist, \underline{Presbyterian}, \underline{Catholic}, \underline{Protestant}, \underline{Christian}} & Welsh,  Scots, Scottish, \underline{British}, Cornish \\ \hline

%Germany     & \multicolumn{1}{l|}{Buddhist, Muslim, \underline{Christian}, Jewish, \underline{Evangelical}}        & Sorbian, \underline{Caucasian}, Frisian, Kurdish, Danish        \\ \hline
\end{tabular}}
\caption{The top 5 identities that are most biased against in the religion and ethnicity sensitives attributes in different regions. These identities are acquired by the average $SOS_{MLM}$ bias scores across all the MLMs in the corresponding language to the region. The \underline{Underlined-text} indicate dominant identities. The rest of the identities are marginalized.}
\label{tab:top-biased-against-identities}
\vspace{-2mm}
\end{table}
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.7\textwidth}
    \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/Egypt/Summarized_SOS_bias_scores_Egypt_boxplot.png}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.7\textwidth}
     \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/Arab_countries/Summarized_SOS_bias_scores_MSA_boxplot.png}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.7\textwidth}
     \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/Germany/Summarized_SOS_bias_scores_Germany_boxplot.png}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.7\textwidth}
     \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/US/Summarized_SOS_bias_scores_US_boxplot.png}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.7\textwidth}
     \centering
         \includegraphics[width=\textwidth]{figures/MLM_results/UK/Summarized_SOS_bias_scores_UK_boxplot.png}
     \end{subfigure}
        \caption{Distribution of the $SOS_{MLM}$ bias scores for the different genders of each Marginalized and Dominant identity in Egypt, the UK and Germany.}
 \label{fig:sos_bias_scores_genders_all_results}
\end{figure}


\FloatBarrier
\subsection{Detailed SOS bias scores for the different regions}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Egypt/SOS bias scores for AraAlBERT(Egypt).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in AraALBERT model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
 \centering
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Egypt/SOS bias scores for AraBART(Egypt).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in AraBART model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
 \centering
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Egypt/SOS bias scores for AraBERT(Egypt).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in AraBERT model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
 \centering
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Egypt/SOS bias scores for XML_Roberta(Egypt).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in XML-Roberta model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Arab_countries/SOS bias scores for AraAlBERT(Arab region).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in AraALBERT model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
 \centering
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Arab_countries/SOS bias scores for AraBART(Arab region).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in AraBART model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
 \centering
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Arab_countries/SOS bias scores for AraBERT(Arab region).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in AraBERT model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
 \centering
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Arab_countries/SOS bias scores for XML_Roberta(Arab region).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in XML-Roberta model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
    
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Germany/SOS bias scores for German_BART(Germany).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in German-BART model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
    
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Germany/SOS bias scores for German_BERT(Germany).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in German-BERT model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Germany/SOS bias scores for German-XLM_Roberta(Germany).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in German-XLM-Roberta model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
    
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/Germany/SOS bias scores for XLM_Roberta(Germany).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in XML-Roberta model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/UK/SOS bias scores for ALBERT(UK).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in AlBERT model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
    
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/UK/SOS bias scores for BART(UK).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in BART model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
    
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/UK/SOS bias scores for BERT(UK).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in BERT model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
  
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/UK/SOS bias scores for XML_Roberta(UK).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in XML-Roberta model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
   
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/US/SOS bias scores for ALBERT(US).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in AlBERT model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
   
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/US/SOS bias scores for BART(US).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in BART model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
    
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/US/SOS bias scores for BERT(US).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in BERT model}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h]
   
    \includegraphics[width=0.7\linewidth]{figures/MLM_results/US/SOS bias scores for XML_Roberta(US).png}
    \caption{The SOS bias scores against individual identities (marginalized and dominant) for the different sensitive attributes in XML-Roberta model}
    \label{fig:enter-label}
\end{figure}


